Feature Adaptation for Sparse Linear Regression

Sparse linear regression is a central problem in high-dimensional statistics. We study the correlated random design setting, where the covariates are drawn from a multivariate Gaussian $N(0,\Sigma)$, and we seek an estimator with small excess risk. If the true signal is $t$-sparse, information-theoretically, it is possible to achieve strong recovery guarantees with only $O(t\log n)$ samples. However, computationally efficient algorithms have sample complexity linear in (some variant of) the condition number of $\Sigma$. Classical algorithms such as the Lasso can require significantly more samples than necessary even if there is only a single sparse approximate dependency among the covariates. We provide a polynomial-time algorithm that, given $\Sigma$, automatically adapts the Lasso to tolerate a small number of approximate dependencies. In particular, we achieve near-optimal sample complexity for constant sparsity and if $\Sigma$ has few ``outlier'' eigenvalues. Our algorithm fits into a broader framework of feature adaptation for sparse linear regression with ill-conditioned covariates. With this framework, we additionally provide the first polynomial-factor improvement over brute-force search for constant sparsity $t$ and arbitrary covariance $\Sigma$.

==> expander.tex <==
\section{Dictionary for expander construction}\label{section:expanders}

In this section, we study the covariance matrices generated by the following process:

\begin{definition}[Expander construction for $\Sigma$]\label{def:expander-sigma}
Fix $n,k \in \NN$ and $\epsilon \geq 0$, and let $M: n/100 \times n$ be a random matrix with i.i.d. Bernoulli entries $\Ber(k/n)$. Define $\Sigma := \epsilon I + \Proj_{\ker(M)}$.
\end{definition}

For $\epsilon$ very small (e.g. $1/\poly(n)$), this matrix is not only ill-conditioned but also has many sparse dependencies \--- one for each row of $M$. As a result, when the ground truth regressor is some $M_i$ and covariates are drawn from $N(0,\Sigma)$, then Lasso fails at exact recovery (given noiseless samples) unless it has a nearly linear number of samples. In fact, it can be shown that (with high probability over the random choice of matrix $M$) for any pre-processing step that applies a change-of-basis, Lasso still fails \cite{kelner2021power, kelner2022distributional}. This makes $\Sigma$ a plausible ``hard example'' for sparse linear regression with correlated random design.

From the perspective of dictionaries, it can be seen that with high probability, the standard basis is \emph{not} an efficient dictionary for $\Sigma$, because the $M_i$'s tend to be uncorrelated with the standard basis vectors under the $\Sigma$-inner product (we will formally prove this as a by-product of a later result in this section). The goal of this section is to show that nonetheless $\Sigma$ does have an efficient dictionary, namely $\{e_1,\dots,e_n,M_1,\dots,M_{n/100}\}$. We prove this only for a restricted class of signals (but conjecture that this is only a limitation of our techniques, and the same dictionary should work for all sparse signals). Specifically, we make the following definition:

\begin{definition}
Let $n,B \in \NN$ and $\CW \in \RR^n$. Let $\Sigma: n \times n$ be a positive semi-definite matrix. A set $\{D_1,\dots,D_N\} \subseteq \RR^n$ is a $(\CW, B)$-$\ell_1$-representation for $\Sigma$ if for any vector $v \in \CW$ there is some $\alpha \in \RR^N$ with $v = \sum_{i=1}^N \alpha_i D_i$ and $$\sum_{i=1}^N |\alpha_i| \cdot \norm{D_i}_\Sigma \leq B \cdot \norm{v}_\Sigma.$$
\end{definition}

With this notation, the original definition of $(t,B)$-$\ell_1$-representability (Definition~\ref{def:l1-rep}) corresponds to setting $\CW := B_0(t)$, the set of $t$-sparse vectors in $\RR^n$. For technical reasons, in this section we are only able to handle integral signals; for any $R \leq \log^{30}(n)$, we will prove that with high probablity $\Sigma$ has a $(\CW_R, R\sqrt{k})$-$\ell_1$-representation, where $\CW_R := \{v \in \mathbb{Z}^n: \norm{v}_1 \leq R\}$.

\paragraph{Graph-theoretic notation \& probabilistic bounds.} The covariance matrix $\Sigma$ defined above is called the expander construction because $M$ can be interpreted as the adjacency matrix of a bipartite graph $G(M)$, and one of the key properties that enables the hardness results of \cite{kelner2021power, kelner2022distributional} is that, with high probability, $G(M)$ is a (bipartite) expander. In our proof we will use related properties (e.g. that $G(M)$ is locally tree-like). We start by formalizing the graph theoretic notation.

\begin{definition}\label{def:m-graph}
Define a bipartite graph $G(M)$ with vertex set $V = I \sqcup J$, where $I = [n]$ and $J = [n/100]$, and with edge set $$\{(i,j) \in I \times J: M_{ji} = 1\}.$$ For any $v \in V$ and $r \geq 0$, let $N_r(v) \subseteq V$ be the set of vertices at distance at most $r$ from $v$ (so $N_0(v) = \{v\}$ and so forth), and let $\partial N_r(v) := N_r(v) \setminus N_{r-1}(v)$. Note that for any $i \in I$, if $r$ is even then $\partial N_r(i) \subseteq I$ and $\partial N_{r+1}(i) \subseteq J$.
\end{definition}

The proof that $\Sigma$ has an $\ell_1$-representation will hold with high probability over the randomness of $M$. In this lemma, we collect the four probabilistic events that we will need, and show that they indeed hold with high probability.

\begin{lemma}\label{lemma:expander-props}
With the setup of Definitions~\ref{def:expander-sigma} and~\ref{def:m-graph}, let $n,k \in \NN$ satisfy $\Omega(\log^5 n) \leq k \leq n^{o(1/\log \log n)}$. Then for any constant $\alpha > 0$, with probability $1-o(1)$, the following properties all hold:
\begin{enumerate}[label=(\alph*)]
    \item For all $i \in I$ it holds that $(1-\alpha)k/100 \leq |\partial N_1(i)| \leq (1+\alpha)k/100$.
    \item For every $j \in J$ it holds that $(1-\alpha)k \leq |\partial N_1(j)| \leq (1+\alpha)k$.
    \item \textbf{(tree-likeness)} Pick any $i_0 \in I$ and even integer $r \in [0, 100\log \log n]$. For any $j \in \partial N_{r+1}(i_0)$:
    \begin{enumerate}[label=(\roman*)]
    \item $\#\{i \in \partial N_1(j) \setminus N_r(i_0): |N_1(i) \cap N_{r+1}(i_0)| > 1\} \leq 2$.
    \item $|\partial N_1(j) \cap N_r(i_0)| \leq 2.$ %Then for all $i,j \in [n] \cup [n/100]$ and every $r \leq 100\log \log n$, if $j \not \in N_r(i)$ then $|N_1(j) \cap N_r(i)| \leq 2$.
    \end{enumerate}
    \item $C_1\sqrt{k} \leq \sigma_\text{min}(M^\t) \leq \sigma_\text{max}(M^\t) \leq C_2\sqrt{k}$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $E$ be the event that Properties (a) and (b) hold. By standard Chernoff bounds and the fact that $k = \Omega(\log n)$, we can obtain the bound $\Pr[E] \geq 1 - 1/n^2$. Property (d) follows from Theorems~1.1 and~1.2 in \cite{gotze2022largest}. It remains to prove that Property (c) holds with probability $1 - o(1)$.

For any $i_0 \in I$, even integer $r \in [0,100\log\log n]$, and $j \in J$, let $E(i_0,r,j)$ be the event that $j \in \partial N_{r+1}(i_0)$ but $\#\{i \in \partial N_1(j): |N_1(i) \cap N_{r+1}(i_0)| > 1\} > 2$. Let $E(i_0,r) = \cup_j E(i_0,r,j)$. Let $F(i_0,r,j)$ be the event that $j \in \partial N_{r+1}(i_0)$ but $|\partial N_1(j) \cap N_r(i_0)| > 2$. Let $F(i_0,r) = \cup_j F(i_0,r,j)$.

\textit{[Proof of (c-i)].} Fix $i_0 \in I$. Note that the random graph $G(M)$ can be equivalently constructed by the following ``breadth-first search'' process. Sample the random variables $\{M_{ji_0}: j \in J\}$ (independently and identically from $\Ber(t/n)$. This determines $N_1(i_0)$. Then sample the random variables $\{M_{ji}: j \in \partial N_1(i_0), i \in I \setminus N_1(i_0)\}$, which determines $N_2(i_0)$. Then sample the random variables $\{M_{ji}: i \in \partial N_2(i_0), j \in J \setminus N_2(i_0)\}$, which determines $N_3(i_0)$, and so on. In general, at step $r$ (for $r$ even), sample the random variables $\{M_{ji}: j \in \partial N_{r-1}(i_0), i \in I \setminus N_{r-1}(i_0)\}$, and for $r$ odd, sample the random variables $\{M_{ji}: i \in \partial N_{r-1}(i_0), j \in J \setminus N_{r-1}(i_0)\}$.

Now also fix an even integer $r \in [0, 100\log\log n]$, and condition on the randomness that determines $N_{r+1}(i_0)$. Suppose that $|N_{r+1}(i_0)| \leq (2k)^{r+2}$ (note that this holds in event $E$). The random sets $\{\partial N_1(j) \setminus N_r(i_0): j \in \partial N_{r+1}(i_0)\}$ are independent and identically distributed: each set $\partial N_1(j) \setminus N_r(i_0)$ is a subset of $I \setminus N_{r+1}(i_0)$, where every element of the latter set is included in $\partial N_1(j)$ with probability $t/n$. Fix $j \in \partial N_{r+1}(i_0)$, and condition on all the other sets, i.e. $\{\partial N_1(j') \setminus N_r(i_0): j' \in \partial N_{r+1}(i_0) \setminus \{j\}\}$. Suppose that each of these sets has size at most $2k$ (note that this holds in event $E$). Any $i \in I$ such that $N_1(i) \cap N_{r+1}(i_0) \not \subseteq \{j\}$ either is contained in $N_{r+1}(i_0)$ or is contained in one of these sets $\partial N_1(j') \setminus N_r(i_0)$. Thus, $$\#\{i \in I: N_1(i) \cap N_{r+1}(i_0) \not \subseteq \{j\}\} \leq (2k)^{r+3}.$$
Now consider the randomness determining the set $\partial N_1(j) \setminus N_r(i_0)$. Each $i \in I$ is included with probability at most $k/n$, but if $|N_1(i) \cap N_{r+1}(i_0)| > 1$ then necessarily $N_1(i) \cap N_{r+1}(i_0) \not \subseteq \{j\}$. So $$\Pr[\#\{i \in \partial N_1(j) \setminus N_r(i_0): |N_1(i) \cap N_{r+1}(i_0)| > 1\} \geq 3] \leq \left(\frac{k}{n}\right)^3 \cdot (2k)^{3(r+3)}.$$
This bound holds for any choice of the conditioned variables that does not make $E$ false. Thus, taking a union bound over $j \in \partial N_{r+1}(i_0)$, $$\Pr[E \cap E(i_0,r)] \leq \left(\frac{k}{n}\right)^3 \cdot (2k)^{3(r+3)} \cdot (2k)^{r+2} \leq \frac{1}{n^{3 - o(1)}}$$
where the last inequality uses that $k = n^{o(1/\log \log n)}$. Finally, by a union bound over $i_0$ and $r$, we get $$\Pr[E \cap \cup_{i_0,r} E(i_0,r)] \leq \frac{1}{n^{2 - o(1)}}.$$
Since $\Pr[E] = 1 - o(1)$, this means that $\Pr[\cup_{i_0,r} E(i_0,r)] = o(1)$.

\textit{[Proof of (c-ii)].} Fix $i_0 \in I$ and an even integer $r \in [0, 100\log \log n]$. Condition on the randomness that determines $N_r(i_0)$. The random sets $\{\partial N_1(i) \setminus N_r(i_0): i \in \partial N_r(i_0)\}$ are independent and identically distributed; each set $\partial N_1(i) \setminus N_r(i_0)$ is a subset of $J \setminus N_r(i_0)$, where every element of the latter set is included in $\partial N_1(i) \setminus N_r(i_0)$ with probability $k/n$. For any $j \in J \setminus N_r(i_0)$, the probability that it's included in more than $2$ of these sets is therefore at most $(k/n)^3 \cdot |\partial N_r(i_0)|^3$, which in event $E$ is at most $1/n^{3 - o(1)}$. Thus, by a union bound over $j \in J$, we get $$\Pr[E \cap F(i_0,r)] \leq \frac{1}{n^{2-o(1)}}.$$
Finally, union bounding over $i_0$ and $r$ and using the fact that $\Pr[E] = 1 - o(1)$ shows that $\Pr[\cup_{i_0,r} F(i_0,r)] = o(1)$.
\end{proof}

We can now simply assume that properties (a)-(d) all hold; we will show that in this event, $\Sigma$ has an $\ell_1$-representation $\{e_1,\dots,e_n,M_1,\dots,M_{n/100}\}$ (at least, with respect to bounded integer-valued vectors). The key step of the proof is the following lemma. Any vector $v$ that is far from $\vspan(M)$ has variance $\norm{v}_\Sigma = \Omega(\norm{v}_2)$, and therefore is efficiently representable using the standard basis vectors. Thus, we are only concerned about sparse vectors that are near $\vspan(M)$. Obviously, these include $\{M_1,\dots,M_{n/100}\}$ and sparse linear combinations thereof; we would like to show that this is essentially everything. It's unclear how to directly prove such a fact, but one approach is to show that we can always find some $M_i$ to add/subtract from $v$ in such a way that progress is made. To this end, the following lemma shows that any sparse vector $v$ near $\vspan(M)$ (relative to $\norm{v}_\infty$) must have sign vector either (strict) majority $+1$'s or (strict) majority $-1$'s on the support of some $M_i$.

\begin{lemma}\label{lemma:sign-agreement}
Suppose that $M: n/100 \times n$ is a binary matrix satisfying Properties (a)-(d) from the above lemma with $\alpha = 0.01$. For any nonzero $v \in \RR^n$ with $\norm{v}_\infty \geq 3\dist(v, \vspan M)$ and $\norm{v}_\infty \geq \norm{v}_2 \cdot (\log n)^{-30}$, there is some $j \in [n/100]$ such that $$\max(\#\{i \in \partial N_1(j): v_i > 0\}, \#\{i \in \partial N_1(j): v_i < 0\}) > \frac{k}{2}.$$ %$\langle M_j, \sign(v) \rangle \neq 0$.
\end{lemma}

\begin{proof}
Let $(N_r(v))$ be the neighborhood sets for the bipartite graph $G(M)$ as defined previously. Pick nonzero $v \in \RR^n$ with $\delta := \dist(v,\vspan M)$ and $\norm{v}_\infty \geq 3\delta$. Suppose that the lemma's conclusion is false, i.e. for every $j \in J$ it holds that the set $\{i \in \partial N_1(j): v_i > 0\}$ has size at most $k/2$, and the set $\{i \in \partial N_1(j): v_i < 0\}$ has size at most $k/2$.

Let $z \in \RR^J$ be such that $\norm{v - M^\t z}_2 = \delta$. Also pick $i_0 \in \argmax_{i \in I} |v_i|$. For any integer $r \geq 0$ let $I_r \subseteq I$ be defined as $I \cap N_r(i_0)$, and let $J_r \subseteq J$ be defined as $J \cap N_r(i_0)$ (so that e.g. $J_0 = \emptyset$). We argue by induction that for all even integers $r \in [0, 100\log\log n]$ it holds that $\sum_{i \in I_r} (v - M_{J_r}^\t z_{J_r})_i^2 \geq (9/4)^r \norm{v}_\infty^2$. 

Indeed, for $r=0$ the left-hand side and right-hand side are both equal to $v_{i_0}^2$. Now suppose that the claim holds for some $r\geq 0$; we prove it for $r+2$. We know that $\norm{(v - M^\t z)_{I_r}}_2 \leq \norm{v - M^\t z}_2 = \delta$ but $\norm{(v - M_{J_r}^\t z_{J_r})_{I_r}}_2 \geq (3/2)^r \norm{v}_\infty$. Thus, by the triangle inequality and the bound $\delta \leq \norm{v}_\infty/3$, $$\norm{(M^\t z - M_{J_r}^\t z_{J_r})_{I_r}}_2 \geq (3/2)^r \norm{v}_\infty - \delta \geq (3/2)^{r-1} \norm{v}_\infty.$$ 
Define $K := J_{r+2} \setminus J_r$. Since $(M^\t z)_i = (M_K^\t z_K)_i + (M_{J_r}^\t z_{J_r})_i$ for all $i \in I_r$, we have that 
\begin{equation}\norm{(M_K^\t z_K)_{I_r}}_2 = \norm{(M^\t z - M_{J_r}^\t z_{J_r})_{I_r}}_2 \geq (3/2)^{r-1} \norm{v}_\infty.\label{eq:k-norm-lb}\end{equation} Pick any $i \in I_r$; observe that we can write 
\begin{equation} (M_K^\t z_K)_i = \sum_{j \in K \cap \partial N_1(i)} z_j.\label{eq:ki-sum}
\end{equation}
For each $j \in K \cap \partial N_1(i)$ define $S_{i,j} \subseteq [n]$ as $$S_{i,j} = \{s \in \partial N_1(j): v_s z_j \leq 0 \text{ and } N_1(s) \cap N_{r+1}(i_0) = \{j\}\}.$$
By Property (b), $|\partial N_1(j)| \geq 0.99k$. By the assumption made at the beginning of the proof, $$\#\{s \in N_1(j): v_s z_j > 0\} \leq k/2.$$
By Property (c), $$\#\{s \in \partial N_1(j): N_1(s) \cap N_{r+1}(i_0) \neq \{j\}\} \leq 4.$$ Thus, $|S_{i,j}| \geq 0.99k - k/2 - 4 \geq k/3$. Also, for any $s \in S_{i,j}$, it holds that $$(v - M_{J_{r+2}}^\t z_{J_{r+2}})_s^2 = \left(v_s - \sum_{j' \in J_{r+2} \cap N_1(s)} z_{j'}\right)^2 = (v_s - z_j)^2 \geq z_j^2$$ where the second equality uses the fact that $J_{r+2} = J_{r+1} = J \cap N_{r+1}(i_0)$ so (since $s \in S_{i,j}$) in fact $J_{r+2} \cap N_1(s) = \{j\}$; the inequality uses the fact that $v_sz_j \leq 0$. Thus, we get
\begin{align}
\sum_{j \in K \cap \partial N_1(i)} \sum_{s \in S_{i,j}} (v - M_{J_{r+2}}^\t z_{J_{r+2}})_s^2 
&\geq (k/3) \sum_{j \in K \cap \partial N_1(i)} z_j^2 \notag \\
&\geq \frac{k}{3|K \cap \partial N_1(i)|}\left(\sum_{j \in K \cap \partial N_1(i)} z_j\right)^2 \tag{Cauchy-Schwarz}\\
&\geq \frac{k}{3(1.01k/100)} (M_K^\t z_K)_i^2\notag
\end{align}
using (\ref{eq:ki-sum}) and the degree bound $|\partial N_1(i)| \leq 1.01k/100$ from Property (a). Summing over $i \in I_r$ and applying (\ref{eq:k-norm-lb}) it follows that
\begin{align}
(\star)\quad \sum_{i \in I_r} \sum_{j \in K \cap \partial N_1(i)} \sum_{s \in S_{i,j}} (v - M_{J_{r+2}}^\t z_{J_{r+2}})_s^2 
&\geq \frac{100}{3.03}\norm{(M_K^\t z_K)_{I_r}}_2^2 \notag \\
&\geq \frac{100}{3.03} (9/4)^{r-1} \norm{v}_\infty^2.\notag
\end{align}
We compare the left-hand side with the quantity we want to lower bound: $$(\dagger) \quad \sum_{i \in I_{r+2}} (v - M_{J_{r+2}}^\t z_{J_{r+2}})_i^2.$$
For any $(i,j,s)$ in ($\star$), we have $j \in J_{r+1}$ so $s \in I_{r+2}$, which means that $(v - M_{J_{r+2}}^\t z_{J_{r+2}})_s^2$ appears in ($\dagger$). Moreover, suppose that $s$ appears multiple times in ($\star$), so there is also some $(i',j',s)$. We have $j \in N_1(s) \cap N_{r+1}(i_0)$ but also $j' \in N_1(s) \cap N_{r+1}(i_0)$, so $j = j'$ (by definition of $S_{i,j}$). But now for every $(i',j,s)$ that appears in the sum, we have $i' \in N_1(s) \cap N_r(i_0)$. By Property (c), the number of such $i'$ is at most $2$. Thus, $(v - M_{J_{r+2}}^\t z_{J_{r+2}})_s^2$ appears at most twice in ($\star$). We conclude that
\begin{align*}
\sum_{i \in I_{r+2}} (v - M_{J_{r+2}}^\t z_{J_{r+2}})_i^2 
&\geq \frac{1}{2}\sum_{i \in I_r} \sum_{j \in K \cap \partial N_1(i)} \sum_{s \in S_{i,j}} (v - M_{J_{r+2}}^\t z_{J_{r+2}})_s^2 \\
&\geq \frac{50}{3.03} (9/4)^{r-1} \norm{v}_\infty^2 \\
&\geq (9/4)^{r+2} \norm{v}_\infty^2.
\end{align*}
This completes the induction. But now taking $r = 100\log\log n$, we get 
\begin{align*}
\norm{v - M_{J_r}^\t z_{J_r}}_2^2
&\geq \sum_{i \in I_r} (v - M_{J_r}^\t z_{J_r})_i^2 \\
&\geq (9/4)^{100\log\log n} \norm{v}_\infty^2 \\
&\geq \norm{v}_\infty^2 \cdot (\log n)^{100} \\
&\geq \norm{v}_2^2 \cdot (\log n)^{40}.
\end{align*}
But by the singular value bounds, we have
\begin{align*}
\norm{M_{J_r}^\t z_{J_r}}_2 
&\leq C_2 \sqrt{k}\norm{z_{J_r}}_2 \\
&\leq C_2\sqrt{k} \norm{z}_2 \\
&\leq C_2 C_1^{-1} \norm{M^\t z}_2 \\
&\leq C_2 C_1^{-1} (\norm{v}_2 + \dist(v, \vspan M)) \\
&\leq (2C_2/C_1) \norm{v}_2
\end{align*}
so in fact $$\norm{v - M_{J_r}^\t z_{J_r}}_2 \leq (1 + 2C_2/C_1)\norm{v}_2$$ which is a contradiction for large $n$.
\end{proof}

A by-product of (a very special case of) the above lemma is a proof that the standard basis is not an efficient dictionary for $\Sigma$ when $\epsilon$ is small (even restricted to sparse $\{-1,0,1\}$-valued signals).

\begin{corollary}
With the setup of Definition~\ref{def:expander-sigma}, let $n,k \in \NN$ satisfy $\Omega(\log^5 n) \leq k \leq n^{o(1/\log \log n)}$. Then with probability $1-o(1)$, for any $\alpha > \sqrt{\epsilon}$, the set $\{e_1,\dots,e_n\}$ is \emph{not} a $(\CW_1, \alpha)$-dictionary for $\Sigma$.
\end{corollary}

\begin{proof}
Suppose that $M$ satisfies Properties (a)-(d) of Lemma~\ref{lemma:expander-props}; by that lemma, this event holds with probability $1-o(1)$. 

Fix $j \in [n/100]$ and pick any $i \in [n]$. Then $|\langle e_i, M_j\rangle_\Sigma| = |\epsilon\langle e_i,M_j\rangle| \leq \epsilon$ and $\norm{M_j}_\Sigma = \sqrt{\epsilon}\norm{M_j}_2 \geq \sqrt{\epsilon \cdot 1.01k}$. Finally, $\norm{e_j}_\Sigma \geq \dist(e_j, \vspan M)$. If $\dist(e_j,\vspan M) \leq 1/3$ then by Lemma~\ref{lemma:sign-agreement}, there is some $j' \in [n/100]$ such that either $\#\{i \in \partial N_1(j'): e_{ji} > 0\}$ or $\#\{i \in \partial N_1(j'): e_{ji} < 0\}$ exceeds $k/2$. But $e_j$ is a standard basis vector, so both of these sets have size at most $1$. Since $k \gg 2$ this is a contradiction, so in fact $\dist(e_j,\vspan M) \leq 1/3$. We conclude that $|\langle e_i, M_j\rangle_\Sigma| \leq \sqrt{\epsilon} \norm{e_i}_\Sigma \norm{M_j}_\Sigma$. Since this holds for all $i \in [n]$, and $M_j \in \CW_1$, we get that $\{e_1,\dots,e_n\}$ is not a $(\CW_1, \alpha)$-dictionary for $\Sigma$ for any $\alpha > \sqrt{\epsilon}$.
\end{proof}

But using the full strength of Lemma~\ref{lemma:sign-agreement}, we can actually show that the dictionary $\CD := \{e_1,\dots,e_n,M_1,\dots,M_{n/100}\}$ is an efficient $\ell_1$-representation for $\Sigma$ (restricted to bounded integer signals). By the same argument as Lemma~\ref{lemma:l1rep-to-covering}, this also implies that every bounded integer signal correlates with some element of $\CD$ under the $\Sigma$-inner product.

\begin{theorem}
With the setup of Definition~\ref{def:expander-sigma}, let $n,k \in \NN$ satisfy $\Omega(\log^5 n) \leq k \leq n^{o(1/\log\log n)}$. Let $R>0$ satisfy $R \leq (\log n)^{30}$. Then with probability $1-o(1)$ it holds that $\{e_1,\dots,e_n,M_1,\dots,M_{n/100}\}$ is a $(\CW_R, R\sqrt{k})$-$\ell_1$-representation for $\Sigma$.
%Let $\epsilon > 0$ and set $\Sigma := \epsilon I + \Proj_{\ker(M)}$. Under the guarantee of the previous lemma, for every nonzero $v \in \mathbb{Z}^n$ with $\norm{v}_1 \leq R$, there are coefficients $\alpha_{1:n}, \beta_{1:n/100} \in \RR$ such that $$v = \sum_{i =1}^n \alpha_i e_i + \sum_{i=1}^{n/100} \beta_i M_i$$ and the ``cost'' of the linear combination is bounded as $$\sum_{i=1}^n |\alpha_i| \sqrt{\frac{e_i^\t \Sigma e_i}{v^\t\Sigma v}} + \sum_{i=1}^{n/10} |\beta_i| \sqrt{\frac{M_i^\t \Sigma M_i}{v^\t\Sigma v}} \leq R\sqrt{t}.$$
\end{theorem}

\begin{proof}
Suppose that $M$ satisfies Properties (a)-(d) of Lemma~\ref{lemma:expander-props}; by that lemma, this event holds with probability $1-o(1)$. 

Let $v \in \CW_R$. We consider two cases. If $\dist(v,\vspan M) \geq 1/3$, then define $\alpha_{1:n} = v_{1:n}$ and $\beta_{1:n/100} = 0$. We obviously have $v = \sum_{i=1}^n \alpha_i e_i + \sum_{j=1}^{n/100} \beta_j M_j$. Moreover $$\sum_{i=1}^n |v_i| \norm{e_i}_\Sigma \leq \norm{v}_1 \sqrt{1+\epsilon} \leq 3\sqrt{\dist(v,\vspan M)^2 + \epsilon\norm{v}_2^2} = 3\norm{v}_\Sigma$$
which suffices. On the other hand, suppose $\dist(v,\vspan M) \leq 1/3$. Since $\norm{v}_\infty \geq 1$ and $\norm{v}_2 \leq R \leq \norm{v}_\infty (\log n)^{30}$, the conditions of Lemma~\ref{lemma:sign-agreement} are satisfied, so there is some $j \in [n/100]$ so that $v$ has the same sign on strictly more than half the indices in $\supp(M_j)$. Say e.g. that $v$ is positive (and thus at least $1$) on strictly more than half of the indices in $\supp(M_j)$. Now $v - M_j \in \mathbb{Z}^n$ satisfies $\norm{v-M_j}_1 \leq \norm{v}_1 - 1$. If $v = M_j$ then we are done; otherwise $\norm{v-M_j}_\infty \geq 1$. But $\dist(v-M_j, \vspan M) = \dist(v,\vspan M) \leq 1/3$ and $$\norm{v-M_j}_2 \leq \norm{v-M_j}_1 \leq \norm{v}_1 \leq R \leq R\norm{v}_\infty,$$ so we can apply Lemma~\ref{lemma:sign-agreement} to $v-M_j$ and repeat this argument until the residual is zero, at which point we have found coefficients $\beta_{1:n/100} \in \RR$ such that $v = \sum_{i=1}^{n/100} \beta_i M_i$ and $\sum_{i=1}^{n/100} |\beta_i| \leq R$. But then $$\sum_{i=1}^{n/100} |\beta_i| \norm{M_i}_\Sigma \leq R \max_i \norm{M_i}_\Sigma \leq R\sqrt{\epsilon k} \leq R\sqrt{k} \norm{v}_\Sigma$$
as needed.
%Since for every $i$ we have $M_i^\t \Sigma M_i = \epsilon \norm{M_i}_2^2 = \epsilon k$ and $v^\t\Sigma v \geq \epsilon \norm{v}_2^2 \geq \epsilon$, the cost of this representation is at most $R\sqrt{t}$.
\end{proof}





==> outlier_existential.tex <==
\section{Existential dictionary construction for $\Sigma$ with few small eigenvalues}

\note{this doesn't actually strictly improve upon Theorem 1.5 because $d$ appears in the sample complexity, but I think it gets rid of the $\exp(t)$ dependence; proof tbd}

\begin{theorem}[Generalized barycentric spanners, \cite{nzg}]
Fix $n,k \in \NN$ and $\delta>0$. Let $V \subseteq \RR^n$ be a $k$-dimensional subspace, and let $S \subseteq \RR^n$ be a compact set so that $\inf_{v \in V} \norm{x-v}_2 \leq \delta$ for all $x \in S$. Then there are $s_1,\dots,s_{3k+1} \in S$ with the following property: for every $x \in S$, there are some $\alpha_1,\dots,\alpha_{3k+1} \in [-1,1]$ for which $\norm{x - \sum_{i=1}^{3k+1} \alpha_i v_i}_2 \leq (3k+1)\delta$.
\end{theorem}

\begin{theorem}
Let $n,t,d \in \NN$. Let $\Sigma: n \times n$ be a positive semi-definite matrix with eigenvalues $\lambda_1 \leq \dots \leq \lambda_n$. Then $\Sigma$ has a $(t, O(dt)\lambda_n/\lambda_{d+1})$-$\ell_1$-representation of size $O(n + d\log(\lambda_n/\lambda_1))$. 
\end{theorem}

\begin{proof}
Consider the eigendecomposition $\Sigma = \sum_{i=1}^n \lambda_i u_i u_i^\t$. Let $V = \vspan\{u_1,\dots,u_d\}$. For each $\alpha > 0$, let $S(\alpha)$ be the set of $t$-sparse vectors $x \in \RR^n$ with $\norm{x}_2 = 1$ and $\alpha \leq \dist(x, V) \leq 2\alpha$. Let $s_1(\alpha),\dots,s_{3d+1}(\alpha) \in S(\alpha)$ be the vectors guaranteed by the above theorem. Define the dictionary to be
\[ \mathcal{D} := \{e_1,\dots,e_n\} \cup \bigcup_{k=0}^{\lceil \log_2(\lambda_n/\lambda_1)\rceil} \{s_1(2^k\lambda_1),\dots,s_{3d+1}(2^k\lambda_1)\}.\]

\end{proof}
